Approximate solution of two dimensional disc-like systems by one dimensional reduction: an approach through the Green function formalism using the Finite Elements Method

We present a comprehensive study for common second order PDE's in two dimensional disk-like systems and show how their solution can be approximated by finding the Green function of an effective one dimensional system. After elaborating on the formalism, we propose to secure an exact solution via a Fourier expansion of the Green function, which entails to solve an infinitely countable system of differential equations for the Green-Fourier modes that in the simplest case yields the source-free Green distribution. We present results on non separable systems$-$or such whose solution cannot be obtained by the usual variable separation technique$-$on both annulus and disc geometries, and show how the resulting one dimensional Fourier modes potentially generate a near-exact solution. Numerical solutions will be obtained via finite differentiation using FDM or FEM with the three-point stencil approximation to derivatives. Comparing to known exact solutions, our results achieve an estimated numerical relative error below $10^{-6}$.

==> biblio.tex <==
@incollection{NIPS2018_7434,
    title = {Accelerated Stochastic Matrix Inversion:  General Theory and  Speeding up BFGS Rules for Faster Second-Order Optimization},
    author = {Gower, Robert and Hanzely, Filip and Richtarik, Peter and Stich, Sebastian U},
    booktitle = {Advances in Neural Information Processing Systems 31},
    editor = {S. Bengio and H. Wallach and H. Larochelle and K. Grauman and N. Cesa-Bianchi and R. Garnett},
    pages = {1619--1629},
    year = {2018},
    publisher = {Curran Associates, Inc.},
    url = {http://papers.nips.cc/paper/7434-accelerated-stochastic-matrix-inversion-general-theory-and-speeding-up-bfgs-rules-for-faster-second-order-optimization.pdf}
}

@article{PhysRevLett.103.206801,
	title = {Anatomy of Abelian and Non-Abelian Fractional Quantum {Hall} States},
	author = {B. Bernevig and N. Regnault},
	journal = {Phys. Rev. Lett.},
	volume = {103},
	issue = {20},
	pages = {206801},
	numpages = {4},
	year = {2009}
}

@article{PhysRevE.73.010501,
	author = "Y. Burak and H. Orland",
	issue = "1",
	journal = "Phys. Rev. E",
	numpages = "4",
	pages = "010501",
	title = "{Manning condensation in two dimensions}",
	volume = "73",
	year = "2006"
}

@article{cornu:2444,
	author = "F. Cornu and B. Jancovici",
	journal = "J. Chem. Phys.",
	number = "4",
	pages = "2444--2452",
	title = "{The electrical double layer: A solvable model}",
	volume = "90",
	year = "1989"
}

@article{PhysRevA.20.2631,
	Author = {C. Deutsch and H. E. Dewitt and Y. Furutani},
	Issue = {6},
	Journal = {Phys. Rev. A},
	Pages = {2631--2633},
	Title = {Debye thermodynamics for the two-dimensional one-component plasma},
	Volume = {20},
	Year = {1979},
}

@article{doi:10.1142/S0217979293003838,
	author = {G. V. Dunne},
	title = {Slater decomposition of {Laughlin} states},
	journal = {Int. J. Mod. Phys. B},
	volume = {07},
	number = {28},
	pages = {4783-4813},
	year = {1993},
}

@article{choquard1983two,
	author = "Ph. Choquard and P. J. Forrester and E. R. Smith",
	issue = "1",
	journal = "J. Stat. Phys.",
	pages = "13--22",
	title = "{The two-dimensional one-component plasma at $\Gamma$=2: The semiperiodic strip}",
	volume = "33",
	year = "1983"
}

@article{forrester1983two,
	author = "P. J. Forrester and B. Jancovici and E. R. Smith",
	issue = "1",
	journal = "J. Stat. Phys.",
	pages = "129--140",
	title = "{The two-dimensional one-component plasma at $\Gamma$=2: Behavior of correlation functions in strip geometry}",
	volume = "31",
	year = "1983"
}

@article{doi:10.1142/S0217751X94001734,
	author = "P. Di Francesco and M. Gaudin and C. Itzykson and F. Lesage",
	journal = "Int. J. Mod. Phys. A",
	number = "24",
	pages = "4257--4351",
	title = "{Laughlin's wave functions, Coulomb gases and expansions of the discriminant}",
	volume = "09",
	year = "1994"
}

@book{Gradshteyn2007,
	Address = {Amsterdam; Boston; Paris [et al.]},
	Author = {I. S. Gradshteyn and I. M. Ryzhik and A. Jeffrey and D. Zwillinger and Scripta Technica Inc.},
	Isbn = {9780123736376 0123736374 9780123738622 0123738628},
	Publisher = {Elsevier : Academic Press},
	Title = {{Table of integrals, series, and products}},
	Year = {2007}
}

@article{vsamaj2004two,
	author = "L. \ifmmode \check{S}\else \v{S}\fi{}amaj",
	issue = "1-2",
	journal = "J. Stat. Phys.",
	pages = "131--158",
	title = "{Is the Two-Dimensional One-Component Plasma Exactly Solvable?}",
	volume = "117",
	year = "2004"
}

@article{vsamaj1995functional,
	author = "L. \ifmmode \check{S}\else \v{S}\fi{}amaj and J. K. Percus",
	issue = "3-4",
	journal = "J. Stat. Phys.",
	pages = "811--824",
	title = "{A functional relation among the pair correlations of the two-dimensional one-component plasma}",
	volume = "80",
	year = "1995"
}

@article{vsamaj2011counter,
	author = "L. \ifmmode \check{S}\else \v{S}\fi{}amaj and E. Trizac",
	journal = "Eur. Phys. J. E",
	number = "2",
	pages = "1--14",
	title = "{Counter-ions at charged walls: Two-dimensional systems}",
	volume = "34",
	year = "2011"
}

@article{PhysRevE.84.041401,
	author = "L. \ifmmode \check{S}\else \v{S}\fi{}amaj and E. Trizac",
	issue = "4",
	journal = "Phys. Rev. E",
	numpages = "17",
	pages = "041401",
	title = "{Wigner-crystal formulation of strong-coupling theory for counterions near planar charged interfaces}",
	volume = "84",
	year = "2011"
}

@article{PhysRevLett.106.078301,
	author = "L. \ifmmode \check{S}\else \v{S}\fi{}amaj and E. Trizac",
	issue = "7",
	journal = "Phys. Rev. Lett.",
	numpages = "4",
	pages = "078301",
	title = "{Counterions at Highly Charged Interfaces: From One Plate to Like-Charge Attraction}",
	volume = "106",
	year = "2011"
}

@article{0295-5075-100-5-56005,
	author = "L. \ifmmode \check{S}\else \v{S}\fi{}amaj and E. Trizac",
	journal = "Europhys. Lett.",
	number = "5",
	pages = "56005",
	title = "{Ground-state structure of a bilayer Wigner crystal with repulsive dielectric images}",
	volume = "100",
	year = "2012"
}

@article{0295-5075-98-3-36004,
	author = "L. \ifmmode \check{S}\else \v{S}\fi{}amaj and E. Trizac",
	journal = "Europhys. Lett.",
	number = "3",
	pages = "36004",
	title = "{Ground state of classical bilayer Wigner crystals}",
	volume = "98",
	year = "2012"
}

@article{PhysRevB.85.205131,
	author = "L. \ifmmode \check{S}\else \v{S}\fi{}amaj and E. Trizac",
	issue = "20",
	journal = "Phys. Rev. B",
	numpages = "15",
	pages = "205131",
	title = "{Critical phenomena and phase sequence in a classical bilayer Wigner crystal at zero temperature}",
	volume = "85",
	year = "2012"
}

@article{PhysRevLett.46.386,
	author = "B. Jancovici",
	issue = "6",
	journal = "Phys. Rev. Lett.",
	pages = "386--388",
	title = "{Exact Results for the Two-Dimensional One-Component Plasma}",
	volume = "46",
	year = "1981"
}

@book{macdonald1998symmetric,
	title={Symmetric functions and {Hall} polynomials},
	author={I. G. Macdonald},
	year={1998},
	publisher={Oxford university press}
}

@article{doi:10.1021/jp311873a,
	author = {J. P. Mallarino and G. T\'ellez and E. Trizac},
	title = {Counterion Density Profile around Charged Cylinders: The Strong-Coupling Needle Limit},
	journal = {J. Phys. Chem. B},
	volume = {117},
	number = {42},
	pages = {12702-12716},
	year = {2013},
}

@Article{MTT14,
	author = {J.P. Mallarino and E. Trizac and G. T\'ellez},
	title = {The contact theorem for charged fluids: from planar to curved geometries},
	journal = {Mol. Phys.},
        DOI={10.1080/00268976.2015.1008595},
	year = {2015}
  }

@article{manning:924,
	author = "G. S. Manning",
	journal = "J. Chem. Phys.",
	number = "3",
	pages = "924--933",
	title = "{Limiting Laws and Counterion Condensation in Polyelectrolyte Solutions I. Colligative Properties}",
	volume = "51",
	year = "1969"
}

@article{manning:934,
	author = "G. S. Manning",
	journal = "J. Chem. Phys.",
	number = "3",
	pages = "934--938",
	title = "{Limiting Laws and Counterion Condensation in Polyelectrolyte Solutions II. Self-Diffusion of the Small Ions}",
	volume = "51",
	year = "1969"
}

@article{manning:3249,
	author = "G. S. Manning",
	journal = "J. Chem. Phys.",
	number = "8",
	pages = "3249--3252",
	title = "{Limiting Laws and Counterion Condensation in Polyelectrolyte Solutions III. An Analysis Based on the Mayer Ionic Solution Theory}",
	volume = "51",
	year = "1969"
}

@book{mehta2004random,
	Author = {M. L. Mehta},
	Date-Added = {2013-04-15 05:41:01 +0000},
	Date-Modified = {2013-04-15 05:42:12 +0000},
	Edition = {Third Edition},
	Editor = {M. L. Mehta},
	Publisher = {Academic press},
	Title = {Random matrices},
	Year = {2004}
}

@article{PhysRevLett.95.185703,
	author = "A. Naji and R. R. Netz",
	issue = "18",
	journal = "Phys. Rev. Lett.",
	numpages = "4",
	pages = "185703",
	title = "{Counterions at Charged Cylinders: Criticality and Universality beyond Mean-Field Theory}",
	volume = "95",
	year = "2005"
}

@article{PhysRevE.73.056105,
	author = "A. Naji and R. R. Netz",
	issue = "5",
	journal = "Phys. Rev. E",
	numpages = "29",
	pages = "056105",
	title = "{Scaling and universality in the counterion-condensation transition at charged cylinders}",
	volume = "73",
	year = "2006"
}

@article{0305-4470-27-12-026,
	author={T. Scharf and J. Thibon and B. G. Wybourne},
	title={Powers of the Vandermonde determinant and the quantum {Hall} effect},
	journal={J. Phys. A},
	volume={27},
	number={12},
	pages={4211},
	year={1994},
}

@article{PhysRevE.49.5623,
	author = "L. {\ifmmode \check{S}\else \v{S}\fi{}amaj} and J. K. Percus and M. Koles{\'i}k",
	issue = "6",
	journal = "Phys. Rev. E",
	pages = "5623--5627",
	title = "{Two-dimensional one-component plasma at coupling $\Gamma${}=4: Numerical study of pair correlations}",
	volume = "49",
	year = "1994"
}

@article{tellez1999exact,
	author = "G. T{\'e}llez and P. J. Forrester",
	issue = "3-4",
	journal = "J. Stat. Phys.",
	pages = "489--521",
	title = "{Exact Finite-Size Study of the 2D OCP at $\Gamma$=4 and $\Gamma$=6}",
	volume = "97",
	year = "1999"
}

@article{tellez2012expanded,
	author = "G. T{\'e}llez and P. J. Forrester",
	issue = "5",
	journal = "J. Stat. Phys.",
	pages = "824--855",
	title = "{Expanded Vandermonde Powers and Sum Rules for the Two-Dimensional One-Component Plasma}",
	volume = "148",
	year = "2012"
}

@article{PhysRevE.85.011119,
	author = "A. Varghese and S. Vemparala and R. Rajesh",
	issue = "1",
	journal = "Phys. Rev. E",
	numpages = "4",
	pages = "011119",
	title = "{Ensemble equivalence for counterion condensation on a two-dimensional charged disk}",
	volume = "85",
	year = "2012"
}

@article{0305-4470-18-9-023,
	author = "P. J. Forrester",
	journal = "J. Phys. A",
	number = "9",
	pages = "1419",
	title = "{The two-dimensional one-component plasma at $\Gamma$ =2: metallic boundary}",
	volume = "18",
	year = "1985"
}

@article{MT2015,
year={2015},
journal={J. Stat. Phys.},
doi={10.1007/s10955-015-1249-2},
title={Relations among two methods for computing the partition function of the two-dimensional one-component plasma},
author={Mora Grimaldo, J. A. and T\'ellez, G.}
}

@article{Ferrero2014,
	doi = {10.1088/1742-5468/2014/11/p11021},
	url = {https://doi.org/10.1088\%2F1742-5468\%2F2014\%2F11\%2Fp11021},
	year = 2014,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {2014},
	number = {11},
	pages = {P11021},
	author = {Alejandro Ferrero and Gabriel T{\'{e}}llez},
	title = {Screening of an electrically charged particle in a two-dimensional two-component plasma at $\Gamma$ = 2},
	journal = {Journal of Statistical Mechanics: Theory and Experiment},
 	abstract = {We consider the thermodynamic effects of an electrically charged impurity immersed in a two-dimensional two-component plasma, composed of particles with charges ±e, at temperature T, at coupling Γ = e2/(kBT) = 2, confined in a large disk of radius R. In particular, we focus on the analysis of the charge density, the correlation functions and the grand potential. Our analytical results show how the charges are redistributed in the circular geometry considered here. When we consider a positively charged impurity, the negative ions accumulate close to the impurity leaving an excess of positive charge that accumulates at the boundary of the disk. Due to the symmetry under charge exchange, the opposite effect takes place when we place a negative impurity. Both cases in which the impurity charge is an integer multiple of the particle charges in the plasma, ±e, and where a fraction of them are considered, require a slightly different mathematical treatment, showing the effect of the quantization of plasma charges. The bulk and the tension effects in the plasma described by the grand potential are not modified by the introduction of the charged particle. Apart from the effects due to the collapse coming from the attraction between oppositely charged ions, an additional topological term appears in the grand potential, proportional to −n2 ln(mR), with n the dimensionless charge of the particle. This term modifies the central charge of the system, from c = 1 to c = 1 − 6n2, when considered in the context of conformal field theories.}
}	


@Article{Ferrero2007,
author="Ferrero, Alejandro
and T{\'e}llez, Gabriel",
title="Two-Dimensional Two-Component Plasma with Adsorbing Impurities",
journal="Journal of Statistical Physics",
year="2007",
month="Nov",
day="01",
volume="129",
number="4",
pages="759--786",
abstract="We study the behavior of the two-dimensional two-component plasma in the presence of some adsorbing impurities. Using a solvable model, we find analytic expressions for the thermodynamic properties of the plasma such as the n-body densities, the grand potential, and the pressure. We specialize in the case where there are one or two adsorbing point impurities in the plasma, and in the case where there are one or two parallel adsorbing lines. In the former case we study the effective interaction between the impurities, due to the charge redistribution around them. The latter case is a model for electrodes with adsorbing sticky sites on their surface.",
issn="1572-9613",
doi="10.1007/s10955-007-9401-2",
url="https://doi.org/10.1007/s10955-007-9401-2"
}


@article{Schwinger1961,
author = {Schwinger,Julian },
title = {Brownian Motion of a Quantum Oscillator},
journal = {Journal of Mathematical Physics},
volume = {2},
number = {3},
pages = {407-432},
year = {1961},
doi = {10.1063/1.1703727},

URL = { 
        https://doi.org/10.1063/1.1703727
    
},
eprint = { 
        https://doi.org/10.1063/1.1703727
}
}

@Article{Wang2014,
author="Wang, Jian-Sheng
and Agarwalla, Bijay Kumar
and Li, Huanan
and Thingna, Juzar",
title="Nonequilibrium Green's function method for quantum thermal transport",
journal="Frontiers of Physics",
year="2014",
month="Dec",
day="01",
volume="9",
number="6",
pages="673--697",
abstract="This review deals with the nonequilibrium Green's function (NEGF) method applied to the problems of energy transport due to atomic vibrations (phonons), primarily for small junction systems. We present a pedagogical introduction to the subject, deriving some of the well-known results such as the Laudauer-like formula for heat current in ballistic systems. The main aim of the review is to build the machinery of the method so that it can be applied to other situations, which are not directly treated here. In addition to the above, we consider a number of applications of NEGF, not in routine model system calculations, but in a few new aspects showing the power and usefulness of the formalism. In particular, we discuss the problems of multiple leads, coupled left-right-lead system, and system without a center. We also apply the method to the problem of full counting statistics. In the case of nonlinear systems, we make general comments on the thermal expansion effect, phonon relaxation time, and a certain class of mean-field approximations. Lastly, we examine the relationship between NEGF, reduced density matrix, and master equation approaches to thermal transport.",
issn="2095-0470",
doi="10.1007/s11467-013-0340-x",
url="https://doi.org/10.1007/s11467-013-0340-x"
}

@article{Foster2019,
author = {Foster, Samuel and Neophytou, Neophytos},
year = {2019},
month = {06},
pages = {91-98},
title = {Effectiveness of nanoinclusions for reducing bipolar effects in thermoelectric materials},
volume = {164},
journal = {Computational Materials Science},
doi = {10.1016/j.commatsci.2019.04.005}
}


@Misc{zbMATH03187565,
 Author = {L. P. {Kadanoff} and G. {Baym}},
 Title = {{Quantum statistical mechanics. Green's function methods in equilibrium and nonequilibrium problems.}},
 Year = {1962},
 Language = {English},
 HowPublished = {{New York: W. A. Benhamin, Inc. XI, 203 p. (1962).}},
 Zbl = {0115.22901}
}

@Article{Lucarini2018,
author="Lucarini, Valerio",
title="Revising and Extending the Linear Response Theory for Statistical Mechanical Systems: Evaluating Observables as Predictors and Predictands",
journal="Journal of Statistical Physics",
year="2018",
month="Dec",
day="01",
volume="173",
number="6",
pages="1698--1721",
abstract="Linear response theory, originally formulated for studying how near-equilibrium statistical mechanical systems respond to small perturbations, has developed into a formidable set of tools for investigating the forced behaviour of a large variety of systems, including non-equilibrium ones. Mathematically rigorous derivations of linear response theory have been provided for systems obeying stochastic dynamics as well as for deterministic chaotic systems. In this paper we provide a new angle on the problem. We study under which conditions it is possible to perform predictions of the response of a given observable of a forced system, using, as predictors, the response of one or more different observables of the same system. This allows us to bypass the need to know all the details of the acting perturbation. Thus, we break the rigid separation between forcing and response, which is key in linear response theory, and revisit the concept of causality. We find that that not all observables are equally good as predictors when a given forcing is applied. In fact, the surrogate Green function one constructs for predicting the response of an observable of interest using a ``bad'' observable as predictor has support that is not limited to the nonnegative time axis. We explain the mathematical reasons behind the fact that an observable is an inefficient predictor. We derive general explicit formulas that, in absence of such pathologies, allow one to reconstruct the response of an observable of interest to N independent external forcings by using as predictors N other observables, with {\$}{\$} N{\backslash}geq 1 {\$}{\$}N≥1. We provide a thorough test of the theory and of the possible pathologies by using numerical simulations of the paradigmatic Lorenz'96 model. Our results are potentially relevant for problems like the reconstruction of data from proxy signals, like in the case of paleoclimate, and, in general, the analysis of signals and feedbacks in complex systems where our knowledge on the system is limited, as in neurosciences. Our technique might also be useful for reconstructing the response to forcings of a spatially extended system in a given location by looking at the response in a separate location.",
issn="1572-9613",
doi="10.1007/s10955-018-2151-5",
url="https://doi.org/10.1007/s10955-018-2151-5"
}

@article{PhysRevLett.120.240601,
  title = {Exact Confirmation of 1D Nonlinear Fluctuating Hydrodynamics for a Two-Species Exclusion Process},
  author = {Chen, Zeying and de Gier, Jan and Hiki, Iori and Sasamoto, Tomohiro},
  journal = {Phys. Rev. Lett.},
  volume = {120},
  issue = {24},
  pages = {240601},
  numpages = {6},
  year = {2018},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.120.240601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.240601}
}

@article{PhysRevA.98.032509,
  title = {Casimir force for magnetodielectric media},
  author = {Brevik, Iver and Parashar, Prachi and Shajesh, K. V.},
  journal = {Phys. Rev. A},
  volume = {98},
  issue = {3},
  pages = {032509},
  numpages = {12},
  year = {2018},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.98.032509},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.98.032509}
}

@article{PhysRevB.89.245430,
  title = {Statistical properties of electrochemical capacitance in disordered mesoscopic capacitors},
  author = {Xu, Fuming and Wang, Jian},
  journal = {Phys. Rev. B},
  volume = {89},
  issue = {24},
  pages = {245430},
  numpages = {8},
  year = {2014},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.89.245430},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.89.245430}
}
@article{GRATSCH20041005,
title = "Duality and finite elements",
journal = "Finite Elements in Analysis and Design",
volume = "40",
number = "9",
pages = "1005 - 1020",
year = "2004",
issn = "0168-874X",
doi = "https://doi.org/10.1016/j.finel.2003.03.002",
url = "http://www.sciencedirect.com/science/article/pii/S0168874X03001392",
author = "Thomas Grätsch and Friedel Hartmann",
keywords = "Duality, Influence function, Green's function, Projection Theorem, Post-processing",
abstract = "Post-processing in finite element analysis is essentially based on duality techniques: nodal values and point values in general or integrals of stresses are obtained by employing influence functions involving appropriate kernel functions Gih(y,x) which are the projections of the exact kernel functions Gi(y,x) onto the trial space Vh. Duality is therefore, as we want to show, a key concept of finite element methods. Questions of accuracy as well as questions of global and local equilibrium can be answered in this context. To this end we first formulate an Equivalence Theorem which establishes the connection between the finite element solution and the exact solution via Green's first identity. We next show that post-processing is essentially an application of Green's first or second identity. Finally, we formulate a new Projection Theorem which encapsulates the whole theory."
}

@book{Springer2017,
  title = "Finite Element Methods, A Practical Guide",
  author = "Jonathan Whiteley",
  year = "2017",
  publisher = "Springer",
  doi = "10.1007/978-3-319-49971-0",
}

@inproceedings{Gower:2018:ASM:3326943.3327092,
 author = {Gower, Robert M. and Hanzely, Filip and Richt\'{a}rik, Peter and Stich, Sebastian U.},
 title = {Accelerated Stochastic Matrix Inversion: General Theory and Speeding Up BFGS Rules for Faster Second-order Optimization},
 booktitle = {Proceedings of the 32Nd International Conference on Neural Information Processing Systems},
 series = {NIPS'18},
 year = {2018},
 location = {Montr\&\#233;al, Canada},
 pages = {1626--1636},
 numpages = {11},
 url = {http://dl.acm.org/citation.cfm?id=3326943.3327092},
 acmid = {3327092},
 publisher = {Curran Associates Inc.},
 address = {USA},
} 

@Inbook{Adams1996,
author="Adams, Malcolm
and Guillemin, Victor",
title="Fourier Analysis",
bookTitle="Measure Theory and Probability",
year="1996",
publisher="Birkh{\"a}user Boston",
address="Boston, MA",
pages="118--177",
abstract="Let (X, ℱ , $\mu$) be a measure space and let f: X {\textrightarrow} C be a complexvalued function. We can write f(x)= u(x) + iv(x), where u and v are realvalued functions on X and {\%} MathType!MTEF!2!1!+-{\%} feaaguart1ev2aaatCvAUfeBSjuyZL2yd9gzLbvyNv2CaerbuLwBLn{\%} hiov2DGi1BTfMBaeXatLxBI9gBaerbd9wDYLwzYbItLDharqqtubsr{\%} 4rNCHbGeaGqiVu0Je9sqqrpepC0xbbL8F4rqqrFfpeea0xe9Lq-Jc9{\%} vqaqpepm0xbba9pwe9Q8fs0-yqaqpepae9pg0FirpepeKkFr0xfr-x{\%} fr-xb9adbaqaaeGaciGaaiaabeqaamaabaabaaGcbaGaamyAaiabg2{\%} da9maakaaabaGaeyOeI0IaaGymaaWcbeaaaaa!39A9!{\$}{\$}i = {\backslash}sqrt {\{} - 1{\}} {\$}{\$}",
isbn="978-1-4612-0779-5",
doi="10.1007/978-1-4612-0779-5_3",
url="https://doi.org/10.1007/978-1-4612-0779-5_3"
}



@article{moore1931,
author = "Moore, C. N.",
fjournal = "Bulletin of the American Mathematical Society",
journal = "Bull. Amer. Math. Soc.",
month = "07",
number = "7",
pages = "510--511",
publisher = "American Mathematical Society",
title = "Review: H. S. Carslaw, Introduction to the Theory of Fourier's Series and Integrals , and Werner Rogosinski, Fouriersche Reihen",
url = "https://projecteuclid.org:443/euclid.bams/1183494882",
volume = "37",
year = "1931"
}

@inbook{shalev-shwartz_ben-david_2014, place={Cambridge}, title={Stochastic Gradient Descent}, DOI={10.1017/CBO9781107298019.015}, booktitle={Understanding Machine Learning: From Theory to Algorithms}, publisher={Cambridge University Press}, author={Shalev-Shwartz, Shai and Ben-David, Shai}, year={2014}, pages={150–166}}

@book{Montavon:2012:NNT:2480981,
 author = {Montavon, Grégoire and Orr, Geneviéve and Müller, Klaus-Robert},
 title = {Neural Networks: Tricks of the Trade},
 year = {2012},
 isbn = {364235288X, 9783642352881},
 edition = {2nd},
 publisher = {Springer Publishing Company, Incorporated},
} 


@Inbook{Tveito2010,
author="Tveito, Aslak
and Langtangen, Hans Petter
and Nielsen, Bj{\o}rn Frederik
and Cai, Xing",
title="Differential Equations: The First Steps",
bookTitle="Elements of Scientific Computing",
year="2010",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="31--73",
abstract="If you know the characteristics of something today, and you know the laws of change, then you can figure out what the characteristicswill be tomorrow. This is the basic idea of modeling lots of natural processes. Since we know the weather today and we know the equations modeling the changes of the weather, we can predict it some days ahead. We know the heat of an object now and we know the equations describing how heat changes; thus we can predict how warm an object will be later on. This is really at the heart of science and has been so for quite a while. But how do we express change? How do we make these vague statements precise and suitable for computer simulations? We do so by expressing the laws of change in terms of differential equations.",
isbn="978-3-642-11299-7",
doi="10.1007/978-3-642-11299-7_2",
url="https://doi.org/10.1007/978-3-642-11299-7_2"
}

@INPROCEEDINGS{8683847,
author={N. {Loizou} and M. {Rabbat} and P. {Richtárik}},
booktitle={ICASSP 2019 - 2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
title={Provably Accelerated Randomized Gossip Algorithms},
year={2019},
volume={},
number={},
pages={7505-7509},
keywords={distributed algorithms;iterative methods;linear systems;protocols;randomised algorithms;wireless sensor networks;average consensus problem;randomized Kaczmarz method;linear systems;accelerated variants;wireless sensor networks;accelerated randomized gossip algorithms;protocols;gossip iteration;private information exchange;Average Consensus;Gossip Protocols;Kaczmarz Methods;Acceleration;Linear Systems},
doi={10.1109/ICASSP.2019.8683847},
ISSN={},
month={May},}

@incollection{NIPS2014_5355,
title = {Stochastic Gradient Descent, Weighted Sampling, and the Randomized Kaczmarz algorithm},
author = {Needell, Deanna and Ward, Rachel and Srebro, Nati},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {1017--1025},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5355-stochastic-gradient-descent-weighted-sampling-and-the-randomized-kaczmarz-algorithm.pdf}
}

@article{DUHAMEL2007919,
title = "Finite element computation of Green's functions",
journal = "Engineering Analysis with Boundary Elements",
volume = "31",
number = "11",
pages = "919 - 930",
year = "2007",
issn = "0955-7997",
doi = "https://doi.org/10.1016/j.enganabound.2007.04.002",
url = "http://www.sciencedirect.com/science/article/pii/S0955799707000781",
author = "D. Duhamel",
keywords = "Green's function, Periodic structure, Wave, Waveguide, Finite element, Dynamic",
abstract = "Green's functions are important mathematical tools in mechanics and in other parts of physics. For instance, the boundary element method needs to know the Green's function of the problem to compute its numerical solution. However, Green's functions are only known in a limited number of cases, often under the form of complex analytical expressions. In this article, a new method is proposed to calculate Green's functions for any linear homogeneous medium from a simple finite element model. The method relies on the theory of wave propagation in periodic media and requires the knowledge of the finite element dynamic stiffness matrix of only one period. Several examples are given to check the accuracy and the efficiency of the proposed numerical Green's function."
}
@article{TONON2001469,
title = "Green’s functions and boundary element method formulation for 3D anisotropic media",
journal = "Computers & Structures",
volume = "79",
number = "5",
pages = "469 - 482",
year = "2001",
issn = "0045-7949",
doi = "https://doi.org/10.1016/S0045-7949(00)00163-2",
url = "http://www.sciencedirect.com/science/article/pii/S0045794900001632",
author = "Fulvio Tonon and Ernian Pan and Bernard Amadei",
keywords = "Green’s displacements, Green’s stresses, Green’s stress derivatives, Elastic anisotropy, Boundary element method, Stress analysis",
abstract = "The implementation of Wang’s theoretical solution is presented for elastostatic displacement Green’s function for three-dimensional solids of general anisotropy. Excerpts from the authors’ fortran code are included. A numerical algorithm for the calculation of the derivatives of the Green’s displacements and stresses is also introduced. These implementations have been incorporated into a boundary element method (BEM) code developed by the authors. The numerical results of Green’s displacements, stresses and stress derivatives are in perfect agreement with closed-form solutions for transversely isotropic solids. The BEM code results are also in very close agreement with both exact solutions and other BEM formulations, even if coarse mesh discretizations are used."
}

@article{PhysRevB.96.205152,
  title = {Restricted Boltzmann machine learning for solving strongly correlated quantum systems},
  author = {Nomura, Yusuke and Darmawan, Andrew S. and Yamaji, Youhei and Imada, Masatoshi},
  journal = {Phys. Rev. B},
  volume = {96},
  issue = {20},
  pages = {205152},
  numpages = {8},
  year = {2017},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.96.205152},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.96.205152}
}
@article{PhysRevE.96.022131,
  title = {Nonequilibrium thermodynamics of restricted Boltzmann machines},
  author = {Salazar, Domingos S. P.},
  journal = {Phys. Rev. E},
  volume = {96},
  issue = {2},
  pages = {022131},
  numpages = {9},
  year = {2017},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.96.022131},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.96.022131}
}

% Artículos de diferencias finitas


@article{articleJo,
author = {Jo, Gwanghyun and Kwak, Do},
year = {2018},
month = {06},
pages = {},
title = {Geometric multigrid algorithms for elliptic interface problems using structured grids},
journal = {Numerical Algorithms},
doi = {10.1007/s11075-018-0544-9}
}

%http://mathsci.kaist.ac.kr/~dykwak/Research/Preprints/10.1007_s11075-018-0544-9pub.pdf

@article{articleBurger,
author = {Ozis, Turgut and Aksan, E.N. and Özdeş, A.},
year = {2003},
month = {07},
pages = {417-428},
title = {A finite element approach for solution of Burgers’ equation},
volume = {139},
journal = {Applied Mathematics and Computation},
doi = {10.1016/S0096-3003(02)00204-7}
}

@article{LIN20071533,
title = "Finite difference/spectral approximations for the time-fractional diffusion equation",
journal = "Journal of Computational Physics",
volume = "225",
number = "2",
pages = "1533 - 1552",
year = "2007",
issn = "0021-9991",
doi = "https://doi.org/10.1016/j.jcp.2007.02.001",
url = "http://www.sciencedirect.com/science/article/pii/S0021999107000678",
author = "Yumin Lin and Chuanju Xu",
keywords = "Fractional diffusion equation, Spectral approximation, Stability, Convergence",
abstract = "In this paper, we consider the numerical resolution of a time-fractional diffusion equation, which is obtained from the standard diffusion equation by replacing the first-order time derivative with a fractional derivative (of order α, with 0⩽α⩽1). The main purpose of this work is to construct and analyze stable and high order scheme to efficiently solve the time-fractional diffusion equation. The proposed method is based on a finite difference scheme in time and Legendre spectral methods in space. Stability and convergence of the method are rigourously established. We prove that the full discretization is unconditionally stable, and the numerical solution converges to the exact one with order O(Δt2-α+N-m), where Δt,N and m are the time step size, polynomial degree, and regularity of the exact solution respectively. Numerical experiments are carried out to support the theoretical claims."
}

% https://www.sciencedirect.com/science/article/pii/S0021999107000678

% https://www.sciencedirect.com/science/article/pii/0021999183900852

%https://en.wikipedia.org/wiki/Burgers%27_equation

@article{articleIzaian,
author = {Izadian, Jalal and Ranjbar, Nasibeh and Jalili, Maryam},
year = {2013},
month = {01},
pages = {95-100},
title = {The Generalized Finite Difference Method for Solving Elliptic Equation on Irregular Mesh},
volume = {21},
journal = {World Applied Sciences Journal},
doi = {10.5829/idosi.wasj.2013.21.am.1396}
}

% http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.388.3658&rep=rep1&type=pdf

@inproceedings{Perrone1975AGF,
  title={A GENERAL FINITE DIFFERENCE METHOD FOR ARBITRARY MESHES},
  author={Nicholas Perrone and Robert S. Kao},
  year={1975}
}

%https://www.sciencedirect.com/science/article/abs/pii/0045794975900188

@article{article,
author = {Shashkov, Mikhail},
year = {2013},
month = {08},
pages = {},
title = {MImetic Finite Difference Method},
journal = {Journal of Computational Physics}
}

% https://www.researchgate.net/publication/256116076_MImetic_Finite_Difference_Method

@article{KWAK199977,
title = "Multigrid algorithm for cell centered finite difference on triangular meshes1This work was partially supported by KOSEF, contract number 971-0106-342-2.1",
journal = "Applied Mathematics and Computation",
volume = "105",
number = "1",
pages = "77 - 85",
year = "1999",
issn = "0096-3003",
doi = "https://doi.org/10.1016/S0096-3003(98)10094-2",
url = "http://www.sciencedirect.com/science/article/pii/S0096300398100942",
author = "Do Y. Kwak and Hyun J. Kwon and Sungyun Lee",
keywords = "Cell centered methods, Finite volume methods, Multigrid methods, -cycle",
abstract = "We consider a multigrid algorithm for the cell centered difference scheme on triangular meshes using a new prolongation operator. The energy norm of this prolongation is shown to be less than 2. Thus the W-cycle is guaranteed to converge. Numerical experiments show that our operator is better than the trivial injection."
}

% https://pdfs.semanticscholar.org/242f/4ccc2217f4a5488f8fee746cfacbdef75935.pdf

@article{doi:10.1002/num.20001,
author = {Kwak, Do Y. and Lee, Jun S.},
title = {Multigrid algorithm for the cell-centered finite difference method II: discontinuous coefficient case},
journal = {Numerical Methods for Partial Differential Equations},
volume = {20},
number = {5},
pages = {742-764},
keywords = {discontinuous coefficient, cell-centered finite difference methods, finite volume methods, multigrid methods},
doi = {10.1002/num.20001},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/num.20001},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/num.20001},
abstract = {Abstract We consider a multigrid algorithm for the cell centered finite difference scheme with a prolongation operator depending on the diffusion coefficient. This prolongation operator is designed mainly for solving diffusion equations with strong varying or discontinuous coefficient and it reduces to the usual bilinear interpolation for Laplace equation. For simple interface problem, we show that the energy norm of this operator is uniformly bounded by 11/8, no matter how large the jump is, from which one can prove that W-cycle with one smoothing converges with reduction factor independent of the size of jump using the theory developed by Bramble et al. (Math Comp 56 (1991), 1–34). For general interface problem, we show that the energy norm is bounded by some constant C* (independent of the jumps of the coefficient). In this case, we can conclude W-cycle converges with sufficiently many smoothings. Numerical experiment shows that even V-cycle multigrid algorithm with our prolongation works well for various interface problems. © 2004 Wiley Periodicals, Inc. Numer Methods Partial Differential Eq, 2004.},
year = {2004}
}

% https://onlinelibrary.wiley.com/doi/abs/10.1002/num.20001

@article{STEGER1978175,
title = "Coefficient matrices for implicit finite difference solution of the inviscid fluid conservation law equations",
journal = "Computer Methods in Applied Mechanics and Engineering",
volume = "13",
number = "2",
pages = "175 - 188",
year = "1978",
issn = "0045-7825",
doi = "https://doi.org/10.1016/0045-7825(78)90056-7",
url = "http://www.sciencedirect.com/science/article/pii/0045782578900567",
author = "Joseph L. Steger",
abstract = "Implicit finite difference methods for the inviscid fluid conservation law equarions are described. Conservative for coefficient matrices are found which are similar to Jacobian linearization and which reduce the computational work of various implicit schemes for the Euler equations of inviscid fluid flow. Extension of the basic ideas is suggested in order to achieve a quite different computational advantage."
}

% https://www.sciencedirect.com/science/article/pii/0045782578900567

@article{Fornberg1988,
abstract = {Simple recursions are derived for calculating the weights in compact finite difference formulas for any order of derivative and to any order of accuracy on one- dimensional grids with arbitrary spacing. Tables are included for some special cases (of equispaced grids).},
author = {Fornberg, Bengt},
doi = {10.1090/S0025-5718-1988-0935077-0},
file = {:Users/jess/Documents/Mendeley Desktop/Fornberg{\_}1988{\_}Generation of finite difference formulas on arbitrarily spaced grids.pdf:pdf},
issn = {0025-5718},
journal = {Mathematics of Computation},
keywords = {Algorithm,Finite differences,High-order accuracy,Interpolation,Math,Numerical Analysis},
mendeley-tags = {Algorithm,Finite differences,High-order accuracy,Interpolation,Math,Numerical Analysis},
number = {184},
pages = {699--699},
title = {{Generation of finite difference formulas on arbitrarily spaced grids}},
url = {http://www.ams.org/journals/mcom/1988-51-184/S0025-5718-1988-0935077-0/ http://amath.colorado.edu/faculty/fornberg/Docs/MathComp{\_}88{\_}FD{\_}formulas.pdf},
volume = {51},
year = {1988}
}


% https://www.ams.org/journals/mcom/1988-51-184/S0025-5718-1988-0935077-0/S0025-5718-1988-0935077-0.pdf

@article{BENITO20011039,
title = "Influence of several factors in the generalized finite difference method",
journal = "Applied Mathematical Modelling",
volume = "25",
number = "12",
pages = "1039 - 1053",
year = "2001",
issn = "0307-904X",
doi = "https://doi.org/10.1016/S0307-904X(01)00029-4",
url = "http://www.sciencedirect.com/science/article/pii/S0307904X01000294",
author = "J.J. Benito and F. Ureña and L. Gavete",
keywords = "Generalized finite differences, Meshless methods, Moving least squares",
abstract = "In this paper it is possible to appreciate the great efficiency of the generalized finite difference method (GFD), that is to say with an irregular arrangements of nodes, to solve second-order partial differential equations which represent the behaviour of many physical processes. The method solves any type of second-order differential equation, in any type of domain and boundary condition (Dirichlet, Neumann and mixed), and immediately obtains the values of derivatives of the nodes through the application of the formulae in differences obtained. This paper analyses the influences of key parameters of the method, such as the number of nodes of the star, the arrangement of the same, the weight function and the stability parameter in time-dependent problems. This analysis includes solutions obtained for different types of problems, represented by different differential equations, including time-dependent equations and under different boundary conditions."
}

% https://www.sciencedirect.com/science/article/pii/S0307904X01000294


% Citation acá, no se por qué putas no sirve https://www.osti.gov/biblio/4731808

% https://www.osti.gov/biblio/4731808


@book{forsythe2013finite,
  title={Finite Difference Methods for Partial Differential Equations: Applied Mathematics Series},
  author={Forsythe, G.E. and Wasow, W.R.},
  isbn={9781258669256},
  url={https://books.google.com.co/books?id=khZYmwEACAAJ},
  year={2013},
  publisher={Literary Licensing, LLC}
}

% https://pdfs.semanticscholar.org/ed35/16cb8fa489a37805c6c588c56fa38cbc2677.pdf

@article{TRUHLAR1972123,
title = "Finite difference boundary value method for solving one-dimensional eigenvalue equations",
journal = "Journal of Computational Physics",
volume = "10",
number = "1",
pages = "123 - 132",
year = "1972",
issn = "0021-9991",
doi = "https://doi.org/10.1016/0021-9991(72)90094-0",
url = "http://www.sciencedirect.com/science/article/pii/0021999172900940",
author = "Donald G Truhlar",
abstract = "The finite difference boundary value method for obtaining eigenvalues and eigenfunctions of the one-dimensional Schroedinger equation is discussed. The method is noniterative and may be applied to one-dimensional problems on (- ∞, ∞) or to the radial equation on (0, ∞). A computer program which computes the eigenvalues and any desired matrix elements involving the eigenfunctions is available from Quantum Chemistry Program Exchange."
}

% https://www.sciencedirect.com/science/article/pii/0021999172900940

@article{articleJomaa,
author = {Jomaa, Z. and Macaskill, Charlie},
year = {2005},
month = {01},
pages = {488-506},
title = {The embedded finite difference method for the Poisson equation in a domain with an irregular boundary and Dirichlet boundary conditions},
volume = {202},
journal = {Journal of Computational Physics},
doi = {10.1016/j.jcp.2004.07.011}
}

% http://www.maths.usyd.edu.au/u/pubs/publist/preprints/2004/jomaa-19.pdf



% Abramovits

@book{abramowitz+stegun,
  added-at = {2008-06-25T06:25:58.000+0200},
  address = {New York},
  author = {Abramowitz, Milton and Stegun, Irene A.},
  biburl = {https://www.bibsonomy.org/bibtex/223ec744709b3a776a1af0a3fd65cd09f/a_olympia},
  description = {BibTeX - Wikipedia, the free encyclopedia},
  edition = {ninth Dover printing, tenth GPO printing},
  interhash = {d4914a420f489f7c5129ed01ec3cf80c},
  intrahash = {23ec744709b3a776a1af0a3fd65cd09f},
  keywords = {Handbook},
  publisher = {Dover},
  timestamp = {2008-06-25T06:25:58.000+0200},
  title = {Handbook of Mathematical Functions with Formulas, Graphs, and Mathematical Tables},
  year = 1964
}

% Jackson

@book{jackson_classical_1999,
  added-at = {2009-07-03T16:37:22.000+0200},
  address = {New York, {NY}},
  author = {Jackson, John David},
  biburl = {https://www.bibsonomy.org/bibtex/2baac05176a92886bbe1eae5ee72cf234/cernlibrary},
  edition = {3rd ed.},
  interhash = {05096e24942ceab2a2e9f0d35a45183a},
  intrahash = {baac05176a92886bbe1eae5ee72cf234},
  isbn = {9780471309321},
  keywords = {Fields Maxwell SummerStudentReadList09 book collisions electromagnetic electrostatic equations magnetostatics particle physics radiation relativity special waves},
  lccn = {538.3537.8},
  publisher = {Wiley},
  timestamp = {2009-07-24T15:58:21.000+0200},
  title = {Classical electrodynamics},
  url = {http://cdsweb.cern.ch/record/490457},
  year = 1999
}

@article{ALKOFER2001281,
title = "The infrared behaviour of QCD Green's functions: Confinement, dynamical symmetry breaking, and hadrons as relativistic bound states",
journal = "Physics Reports",
volume = "353",
number = "5",
pages = "281 - 465",
year = "2001",
issn = "0370-1573",
doi = "https://doi.org/10.1016/S0370-1573(01)00010-2",
url = "http://www.sciencedirect.com/science/article/pii/S0370157301000102",
author = "Reinhard Alkofer and Lorenz von Smekal",
keywords = "Strong QCD, Green's functions, Confinement, Chiral symmetry breaking, Dyson–Schwinger equations, Bethe-Salpeter equation",
abstract = "Recent studies of QCD Green's functions and their applications in hadronic physics are reviewed. We discuss the definition of the generating functional in gauge theories, in particular, the rôle of redundant degrees of freedom, possibilities of a complete gauge fixing versus gauge fixing in presence of Gribov copies, BRS invariance and positivity. The apparent contradiction between positivity and colour antiscreening in combination with BRS invariance in QCD is considered. Evidence for the violation of positivity by quarks and transverse gluons in the covariant gauge is collected, and it is argued that this is one manifestation of confinement. We summarise the derivation of the Dyson–Schwinger equations (DSEs) of QED and QCD. For the latter, the implications of BRS invariance on the Green's functions are explored. The possible influence of instantons on DSEs is discussed in a two-dimensional model. In QED in (2+1) and (3+1) dimensions, the solutions for Green's functions provide tests of truncation schemes which can under certain circumstances be extended to the DSEs of QCD. We discuss some limitations of such extensions and assess the validity of assumptions for QCD as motivated from studies in QED. Truncation schemes for DSEs are discussed in axial and related gauges, as well as in the Landau gauge. Furthermore, we review the available results from a systematic non-perturbative expansion scheme established for Landau gauge QCD. Comparisons to related lattice results, where available, are presented. The applications of QCD Green's functions to hadron physics are summarised. Properties of ground state mesons are discussed on the basis of the ladder Bethe-Salpeter equation for quarks and antiquarks. The Goldstone nature of pseudoscalar mesons and a mechanism for diquark confinement beyond the ladder approximation are reviewed. We discuss some properties of ground state baryons based on their description as Bethe-Salpeter/Faddeev bound states of quark–diquark correlations in the quantum field theory of confined quarks and gluons."
}

% https://www.sciencedirect.com/science/article/abs/pii/S0370157301000102

@article{LENZI2000503,
title = "Green functions based on Tsallis nonextensive statistical mechanics: normalized q-expectation value formulation",
journal = "Physica A: Statistical Mechanics and its Applications",
volume = "286",
number = "3",
pages = "503 - 517",
year = "2000",
issn = "0378-4371",
doi = "https://doi.org/10.1016/S0378-4371(00)00364-2",
url = "http://www.sciencedirect.com/science/article/pii/S0378437100003642",
author = "E.K. Lenzi and R.S. Mendes and A.K. Rajagopal",
abstract = "In this paper, the Green function theory of quantum many-particle systems recently presented is reworked within the framework of nonextensive statistical mechanics with a new normalized q-expectation values. This reformulation introduces a renormalization of temperature of the earlier theory and a self-consistency condition. The importance of these two features is nontrivial and to emphasize this, we explicitly contrast the maximum entropy density matrices derived for an exactly solvable model based on the two types of the constraints. The linear response theory is also presented, along with its two-particle Green function version. In order to emphasize the importance of the new formalism, we collect here the results where both the formalisms have been used to examine the same set of problems. This reveals clearly that the new formalism is the method of choice because the numerical results are much more physically meaningful than those found in the old version, even though the general features or the answers retain the same characteristics in certain cases. In the case where thermodynamic entities are to be examined as in the case of the q-dependence of Bose–Einstein condensation, the self-consistent requirement in the new formalism is numerically much more subtle, and thus the earlier results are modified as shown in Fig. 1."
}

% https://www.sciencedirect.com/science/article/pii/S0378437100003642

@Article{C5NR01052G,
author ="Schwierz, F. and Pezoldt, J. and Granzner, R.",
title  ="Two-dimensional materials and their prospects in transistor electronics",
journal  ="Nanoscale",
year  ="2015",
volume  ="7",
issue  ="18",
pages  ="8261-8283",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C5NR01052G",
url  ="http://dx.doi.org/10.1039/C5NR01052G",
abstract  ="During the past decade{,} two-dimensional materials have attracted incredible interest from the electronic device community. The first two-dimensional material studied in detail was graphene and{,} since 2007{,} it has intensively been explored as a material for electronic devices{,} in particular{,} transistors. While graphene transistors are still on the agenda{,} researchers have extended their work to two-dimensional materials beyond graphene and the number of two-dimensional materials under examination has literally exploded recently. Meanwhile several hundreds of different two-dimensional materials are known{,} a substantial part of them is considered useful for transistors{,} and experimental transistors with channels of different two-dimensional materials have been demonstrated. In spite of the rapid progress in the field{,} the prospects of two-dimensional transistors still remain vague and optimistic opinions face rather reserved assessments. The intention of the present paper is to shed more light on the merits and drawbacks of two-dimensional materials for transistor electronics and to add a few more facets to the ongoing discussion on the prospects of two-dimensional transistors. To this end{,} we compose a wish list of properties for a good transistor channel material and examine to what extent the two-dimensional materials fulfill the criteria of the list. The state-of-the-art two-dimensional transistors are reviewed and a balanced view of both the pros and cons of these devices is provided."}

% https://pubs.rsc.org/en/content/articlelanding/2015/nr/c5nr01052g#!divAbstract

@article{articleFG,
author = {Fiori, Gianluca and Bonaccorso, Francesco and Iannaccone, Giuseppe and Palacios, Tomas and Neumaier, Daniel and Seabaugh, Alan and Banerjee, Sanjay and Colombo, Luigi},
year = {2014},
month = {10},
pages = {768-779},
title = {Electronics based on two-dimensional materials},
volume = {9},
journal = {Nature Nanotechnology},
doi = {10.1038/nnano.2014.207}
}

% https://pubs.rsc.org/en/content/articlelanding/2015/nr/c5nr01052g#!divAbstract

@article {Novoselov666,
	author = {Novoselov, K. S. and Geim, A. K. and Morozov, S. V. and Jiang, D. and Zhang, Y. and Dubonos, S. V. and Grigorieva, I. V. and Firsov, A. A.},
	title = {Electric Field Effect in Atomically Thin Carbon Films},
	volume = {306},
	number = {5696},
	pages = {666--669},
	year = {2004},
	doi = {10.1126/science.1102896},
	publisher = {American Association for the Advancement of Science},
	abstract = {We describe monocrystalline graphitic films, which are a few atoms thick but are nonetheless stable under ambient conditions, metallic, and of remarkably high quality. The films are found to be a two-dimensional semimetal with a tiny overlap between valence and conductance bands, and they exhibit a strong ambipolar electric field effect such that electrons and holes in concentrations up to 1013 per square centimeter and with room-temperature mobilities of \~{}10,000 square centimeters per volt-second can be induced by applying gate voltage.},
	issn = {0036-8075},
	URL = {https://science.sciencemag.org/content/306/5696/666},
	eprint = {https://science.sciencemag.org/content/306/5696/666.full.pdf},
	journal = {Science}
}

% https://science.sciencemag.org/content/306/5696/666

@article{articleSR,
author = {Sterling, R and Rattanasonti, Hwanjit and Weidt, Seb and Lake, Kimberley and Srinivasan, Palaniyappan and Webster, S and Kraft, Michael and Hensinger, W.},
year = {2014},
month = {04},
pages = {3637},
title = {Fabrication and operation of a two-dimensional ion-trap lattice on a high-voltage microchip},
volume = {5},
journal = {Nature communications},
doi = {10.1038/ncomms4637}
}

% https://www.nature.com/articles/ncomms4637



@article{doi:10.1021/nl0518472,
author = {Flindt, Christian and Mortensen, Niels Asger and Jauho, Antti-Pekka},
title = {Quantum Computing via Defect States in Two-Dimensional Antidot Lattices},
journal = {Nano Letters},
volume = {5},
number = {12},
pages = {2515-2518},
year = {2005},
doi = {10.1021/nl0518472},
    note ={PMID: 16351206},

URL = { 
        https://doi.org/10.1021/nl0518472
    
},
eprint = { 
        https://doi.org/10.1021/nl0518472
    
}

}


@article{articleSF,
author = {Sugino, Fumihiko},
year = {2004},
month = {01},
pages = {},
title = {Super Yang-Mills Theories on the Two-Dimensional Lattice with Exact Supersymmetry},
volume = {403},
journal = {JHEP},
doi = {10.1088/1126-6708/2004/03/067}
}

% https://www.researchgate.net/publication/1988489_Super_Yang-Mills_Theories_on_the_Two-Dimensional_Lattice_with_Exact_Supersymmetry

@article{GAMBOASARAVI1981239,
title = "Path-integral formulation of two-dimensional gauge theories with massless fermions",
journal = "Nuclear Physics B",
volume = "185",
number = "1",
pages = "239 - 253",
year = "1981",
issn = "0550-3213",
doi = "https://doi.org/10.1016/0550-3213(81)90375-8",
url = "http://www.sciencedirect.com/science/article/pii/0550321381903758",
author = "R.E. Gamboa Saraví and F.A. Schaposnik and J.E. Solomin",
abstract = "We study (1 + 1) dimensional gauge theories [with SU(N) and diagonal SU(N) color symmetry] using the functional integral method. We construct an effective lagrangian by performing a change in the fermionic variables, and then investigate relevant phenomena such as the intrinsic Higgs mechanism and color screening."
}

% https://www.sciencedirect.com/science/article/pii/0550321381903758

@article{articlePA,
author = {Perera, Aurélien and Urbic, Tomaz},
year = {2018},
month = {02},
pages = {},
title = {Clustering in complex ionic liquids in two dimensions},
volume = {265},
journal = {Journal of Molecular Liquids},
doi = {10.1016/j.molliq.2018.05.133}
}

% https://www.researchgate.net/publication/323003863_Clustering_in_complex_ionic_liquids_in_two_dimensions

@article{doi:10.1063/1.533014,
author = {Rañada,Manuel F.  and Santander,Mariano },
title = {Superintegrable systems on the two-dimensional sphere S2 and the hyperbolic plane H2},
journal = {Journal of Mathematical Physics},
volume = {40},
number = {10},
pages = {5026-5057},
year = {1999},
doi = {10.1063/1.533014},

URL = { 
        https://doi.org/10.1063/1.533014
    
},
eprint = { 
        https://doi.org/10.1063/1.533014
}}

% https://aip.scitation.org/doi/abs/10.1063/1.533014

@article{doi:10.1063/1.1897183,
author = {Kalnins,E. G.  and Kress,J. M.  and Miller,W. },
title = {Second-order superintegrable systems in conformally flat spaces. I. Two-dimensional classical structure theory},
journal = {Journal of Mathematical Physics},
volume = {46},
number = {5},
pages = {053509},
year = {2005},
doi = {10.1063/1.1897183},

URL = { 
        https://doi.org/10.1063/1.1897183
    
},
eprint = { 
        https://doi.org/10.1063/1.1897183
}}

% https://aip.scitation.org/doi/abs/10.1063/1.1897183

@article{PhysRevD.55.3830,
  title = {Static intervortex forces},
  author = {Speight, J. M.},
  journal = {Phys. Rev. D},
  volume = {55},
  issue = {6},
  pages = {3830--3835},
  numpages = {0},
  year = {1997},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.55.3830},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.55.3830}
}

% https://journals.aps.org/prd/abstract/10.1103/PhysRevD.55.3830 
% https://arxiv.org/pdf/hep-th/9603155.pdf








@article{doi:10.1080/03605302.2010.489629,
author = { Dorina   Mitrea  and  Irina   Mitrea },
title = {On the Regularity of Green Functions in Lipschitz Domains},
journal = {Communications in Partial Differential Equations},
volume = {36},
number = {2},
pages = {304-327},
year  = {2010},
publisher = {Taylor & Francis},
doi = {10.1080/03605302.2010.489629},

URL = { 
        https://doi.org/10.1080/03605302.2010.489629
    
},
eprint = { 
        https://doi.org/10.1080/03605302.2010.489629
    
}

}

    @article {,
    author = {Calderón A.P.},
    author = {Torchinsky A.},
    title = {Parabolic maximal functions associated with a distribution. II},
    journal = {Adv. Math.},
    volume = {24},
    pages = {101},
    year = {1977}
    }

    @article {,
    author = {Dahlberg B.},
    title = {L q -estimates for Green potentials in Lipschitz domains},
    journal = {Math. Scand.},
    volume = {44},
    pages = {149},
    year = {1979}
    }

    @article {,
    author = {Gao W.},
    title = {Layer potentials and boundary value problems for elliptic systems in Lipschitz domains},
    journal = {J. Fun. Anal.},
    volume = {95},
    pages = {377},
    year = {1991}
    }

    @article {,
    author = {Grüter M.},
    author = {Widman K.O.},
    title = {The Green function for uniformly elliptic equations},
    journal = {Manuscripta Math.},
    volume = {37},
    pages = {303},
    year = {1982}
    }

    @article {,
    author = {Jerison D.},
    author = {Kenig C.},
    title = {The inhomogeneous problem in Lipschitz domains},
    journal = {J. Funct. Anal.},
    volume = {130},
    pages = {161},
    year = {1995}
    }

    @article {,
    author = {Mayboroda S.},
    author = {Maz'ya V.},
    title = {Boundedness of the gradient of a solution and Wiener test of order one for the biharmonic equation},
    journal = {Invent. Math.},
    volume = {175},
    pages = {287},
    year = {2009}
    }

    @article {,
    author = {Maz'ya V.},
    author = {Mitrea M.},
    author = {Shaposhnikova T.},
    title = {The Dirichlet problem in Lipschitz domains with boundary data in Besov spaces for higher order elliptic systems with rough coefficients},
    journal = {Journal d'Analyse Mathématique},
    volume = {},
    pages = {},
    year = {}
    }

    @article {,
    author = {Mitrea D.},
    title = {A generalization of Dahlberg&#039;s theorem concerning the regularity of harmonic Green potentials},
    journal = {Trans. AMS},
    volume = {360},
    pages = {3771},
    year = {2008}
    }

    @article {,
    author = {Mitrea D.},
    author = {Mitrea I.},
    title = {General second order, strongly elliptic systems inlow dimensional nonsmooth manifolds},
    journal = {Contemp. Math.},
    volume = {277},
    pages = {61},
    year = {2001}
    }

    @article {,
    author = {Mitrea I.},
    author = {Mitrea M.},
    title = {On the regularity of the green potential for the Laplacian with Robin boundary condition},
    journal = {Integral Methods for Science and Engineering},
    volume = {1},
    pages = {235},
    year = {2010}
    }

    @article {,
    author = {Mitrea I.},
    author = {Mitrea M.},
    author = {Wright M.},
    title = {Optimal estimates for the inhomogeneous problem for the bi-Laplacian in three-dimensional Lipschitz domains},
    journal = {J. Math. Sci.},
    volume = {},
    pages = {},
    year = {}
    }

    @article {,
    author = {Mitrea M.},
    author = {Taylor M.},
    title = {Potential theory on Lipschitz domains in Riemannian manifolds: Sobolev–Besov space results and the Poisson problem},
    journal = {J. Funct. Anal.},
    volume = {176},
    pages = {1},
    year = {2000}
    }

    @article {,
    author = {Nečas J.},
    title = {Sur une méthode pour résoudre les équations aux dérivées partielles du type elliptique, voisine de la variationnelle},
    journal = {Ann. Scuola Norm. Sup. Pisa},
    volume = {3},
    pages = {305},
    year = {1962}
    }

    @article {,
    author = {Shen Z.},
    title = {The L p Dirichlet problem for elliptic systems on Lipschitz domains},
    journal = {Math. Res. Letters},
    volume = {13},
    pages = {143},
    year = {2006}
    }

    @article {,
    author = {Whitney H.},
    title = {Analytic extensions of differentiable functions defined in closed sets},
    journal = {Trans. Amer. Math. Soc.},
    volume = {36},
    pages = {63},
    year = {1934}
    }



